Robust Multimodal 3D Object Detection via Modality-Agnostic Decoding and Proximity-based Modality Ensemble

Recent advancements in 3D object detection have benefited from multi-modal information from the multi-view cameras and LiDAR sensors. However, the inherent disparities between the modalities pose substantial challenges. We observe that existing multi-modal 3D object detection methods heavily rely on the LiDAR sensor, treating the camera as an auxiliary modality for augmenting semantic details. This often leads to not only underutilization of camera data but also significant performance degradation in scenarios where LiDAR data is unavailable. Additionally, existing fusion methods overlook the detrimental impact of sensor noise induced by environmental changes, on detection performance. In this paper, we propose MEFormer to address the LiDAR over-reliance problem by harnessing critical information for 3D object detection from every available modality while concurrently safeguarding against corrupted signals during the fusion process. Specifically, we introduce Modality Agnostic Decoding (MOAD) that extracts geometric and semantic features with a shared transformer decoder regardless of input modalities and provides promising improvement with a single modality as well as multi-modality. Additionally, our Proximity-based Modality Ensemble (PME) module adaptively utilizes the strengths of each modality depending on the environment while mitigating the effects of a noisy sensor. Our MEFormer achieves state-of-the-art performance of 73.9% NDS and 71.5% mAP in the nuScenes validation set. Extensive analyses validate that our MEFormer improves robustness against challenging conditions such as sensor malfunctions or environmental changes. The source code is available at https://github.com/hanchaa/MEFormer

==> rebuttal/sec/apply_pme.tex <==
\noindent\textbf{[Reviewer \#1] Applying PME to other baselines.}
We agree that PME would be also effective for other fusion-based methods as PME alone improves CMT.
However, as shown in Fig. 1 in the main paper, other methods show near 0\% mAP in the camera-only scenario.
In this case, PME cannot utilize the camera modality.
Although MetaBEV shows robust performance in the camera-only scenario, we are not able to apply PME to it because they have not published the code.


==> rebuttal/sec/central_argument.tex <==
%\noindent\textbf{[Review \#1] About the central argument of the paper.}
\noindent\textbf{[Reviewer \#1] Addressing heavy reliance on LiDAR.}
We empirically prove that our MEFormer effectively addresses the LiDAR reliance problem.
%We think our central argument still holds that MEFormer addresses the LiDAR reliance problem.
As mentioned by R1, when LiDAR is missing, a performance drop is inevitable.
However, previous works exhibit a significant degradation, underperforming the same architecture trained with cameras alone.
%the detection task without LiDAR.
% either barely perform the detection task without LiDAR or show lower performance than the same architecture trained with cameras alone.
For example, when LiDAR is missing, CMT performs 1.3\% lower in mAP and NDS compared to CMT-C which is trained with only camera modality.
Furthermore, BEVFusion barely detects objects, showing near `0\%' mAP.
%Some existing methods even show near `0\%' mAP.
This is because they fail to combine useful information from both modalities and rely on LiDAR information.
We address the LiDAR reliance problem by combining useful information from both modalities using MOAD.
As a result, MOAD shows 2\% higher NDS compared to CMT-C when LiDAR is missing.
% Although it is straightforward that LiDAR is more useful than cameras for 3D object detection, many previous works show that camera-only detectors can also perform 3D object detection.
% However, baseline methods do not consider this aspect of the camera modality when fusing the multi-modal information, and they show poor performance without LiDAR information.
% We define this phenomenon as LiDAR reliance problem and propose MOAD and PME that effectively combine useful information from both LiDAR and cameras.

==> rebuttal/sec/detail_explanations.tex <==
\noindent\textbf{[Reviewer \#6] Detailed explanations about characteristics of each modality.}
As discussed in LiStereo\footnote{Zhang, Junming, et al. Listereo: Generate dense depth maps from lidar and stereo imagery. ICRA. 2020. \vspace{-10pt}}, LiDAR has accurate geometric information but its resolution is sparser than the camera, which is vulnerable to distant objects.
On the other hand, the camera has dense information which allows the detection of small and distant objects.
MOAD makes models detect 3D objects solely with cameras which forces image backbone to extract 3D geometric information from multi-view images.
This training strategy enables the model to successfully localize objects using camera modality that LiDAR fails to detect due to its sparsity.
As a result, Table~\ref{pme_gain} shows that MOAD improves 1.1\% mAP compared to CMT which is our baseline.
Note that PME is the module for preventing negative fusion not for extracting geometric information from the camera modality.

==> rebuttal/sec/distance_threshold.tex <==
\noindent\textbf{[Reviewer \#1, \#6] Distance threshold for PME.}
Table~\ref{distance_threshold} shows performance comparison according to distance threshold $d$ in Eq. (9) in the main paper.
PME shows the best performance with $d=2$ and performance degrades as $d$ increases.
It shows that it is important to avoid ensembles with irrelevant boxes.
Table~\ref{hard_and_soft} shows a performance comparison between the hard threshold and soft threshold.
Thanks to the constructive comments from reviewers, we achieve higher performance.
For the soft threshold, we linearly transform box distance and add it to the attention score logit.
This can be formulated as $\hat{d}_{i,j} = s * d_{i, j} + b$, $A_{i,j} = q_i \cdot k_j + \hat{d}_{i,j}$, where $s, b\in\mathbb{R}^1$ are learnable scaler and bias and $d_{i,j}$ is the distance between $i$-th box and $j$-th box. $A_{i, j}$ is the attention score logit and we applied softmax as the attention mechanism.
Note that $\hat{d}_{i, j}$ can be considered as a relative position embedding.
As a result, MEFormer outperforms CMT by 1.0\% in NDS and 1.2\% in mAP.
We appreciate constructive comments and we will include them in the final version.
\input{rebuttal/table/distance_threshold}

==> rebuttal/sec/pme_gain.tex <==
\noindent\textbf{[Reviewer \#1, \#3, \#6] Performance gain by PME.}
The performance gain by PME seems relatively small compared to MOAD in Table 4 of the main paper but this is mainly due to the performance saturation.
%Instead of evaluating PME on top of CMT with MOAD, we evaluate PME directly on CMT. 
%It seems that a small performance improvement by introducing PME to MOAD is due to the performance saturation.
Table~\ref{pme_gain} shows the performance in challenging environments.
Although the performance gap between MOAD and `MOAD with PME' seems marginal, `CMT with PME' shows larger performance improvements compared to CMT and this verifies the effectiveness of PME module in challenging environments.
Specifically, CMT with PME shows 0.5\% NDS improvement in rainy environments and 0.4\% mAP improvement for distant objects.
In addition, Table~\ref{dirt_occlusion} shows that PME also improves performance in a camera malfunction scenario.
Introducing PME to MOAD improves mAP by 0.3\%, and CMT with PME shows a larger mAP gain by 0.6\%.
% Applying PME to the method which performs lower shows larger performance improvements and our argument that PME is effective for robustness still holds.
\input{rebuttal/table/challenging_environments}
\input{rebuttal/table/camera_malfunction}

==> rebuttal/table/camera_malfunction.tex <==
\begin{table}[h]
\centering
\footnotesize
\setlength{\tabcolsep}{15pt}
\begin{tabular}{lcc}
    \toprule
    \multirow{2}{*}[-2pt]{Method} & \multicolumn{2}{c}{Camera Dirt Occlusion} \\
    \cmidrule(lr){2-3}
    & NDS & mAP \\
    \midrule
    \midrule
    CMT         & 69.2 & 63.9 \\
    CMT w/ PME  & 69.6 & 64.5 \\
    \midrule
    MOAD        & 69.7 & 64.3 \\
    MOAD w/ PME & 69.9 & 64.6 \\
    \bottomrule
\end{tabular}
\vspace{-0.8em}
\caption{\textbf{Performance comparison in another camera malfunction scenario.} We add a dirt mask to the same camera in the same scene for all experiments.}
\label{dirt_occlusion}
\vspace{-2.6em}
\end{table}



==> rebuttal/table/challenging_environments.tex <==
\begin{table}[h]
\centering
\footnotesize
% \vspace{-1em}
\begin{tabular}{lcccccc}
    \toprule
    \multirow{2}{*}[-2pt]{Method} & \multicolumn{2}{c}{Night} & \multicolumn{2}{c}{Rainy} & \multicolumn{2}{c}{Distant}\\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
    & NDS & mAP & NDS & mAP & NDS & mAP \\
    \midrule
    \midrule
    CMT         & 46.3 & 42.8 & 73.7 & 70.5 & 52.6 & 42.5\\
    CMT w/ PME  & 46.5 & 43.2 & 74.2 & 70.8 & 52.9 & 42.9\\
    \midrule
    MOAD        & 46.6 & 43.1 & 74.6 & 72.2 & 53.4 & 43.6\\
    MOAD w/ PME & 46.8 & 43.6 & 74.7 & 72.2 & 53.4 & 43.7\\
    \bottomrule
\end{tabular}
\vspace{-1.2em}
\caption{\textbf{Performance gain of PME in challenging environments.}}
\label{pme_gain}
\vspace{-1.0em}
\end{table}

==> rebuttal/table/distance_threshold.tex <==
\begin{table}[h]
\centering
\small
\vspace{-0.8em}
\begin{minipage}{.49\linewidth}
\begin{tabular}{lcc}
    \toprule
    {Method} & {NDS} & {mAP}\\
    \midrule
    \midrule
    $d=1$ & \textbf{73.8} & 71.3 \\
    $d=2$ & \textbf{73.8} & \textbf{71.4} \\
    $d=4$ & 73.7 & 71.3 \\
    $d=\infty$ & 73.6 & 71.2 \\
    \bottomrule
\end{tabular}
\vspace{-1em}
\caption{\textbf{Comparison of distance threshold.}}
\label{distance_threshold}
% \vspace{-1.2em}
\end{minipage}
\begin{minipage}{.49\linewidth}
\begin{tabular}{lcc}
    \toprule
    {Method} & {NDS} & {mAP}\\
    \midrule
    \midrule
    CMT         & 72.9 & 70.3 \\
    MOAD        & 73.7 & 71.3 \\
    PME (hard)  & 73.8 & 71.4 \\
    PME (soft)  & \textbf{73.9} & \textbf{71.5} \\
    \bottomrule
\end{tabular}
\vspace{-1em}
\caption{\textbf{Comparison of hard threshold and soft threshold.}}
\label{hard_and_soft}
\end{minipage}
\vspace{-1.5em}
\end{table}

==> supple/image/supple_qual_dark.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.95\textwidth]{supple/image/supple_qual_dark.pdf}
    \caption{
    \textbf{Qualitative comparison of ours without PME and with PME.}
    Ours without PME fails to localize the motorcycle that the camera-only decoding branch identifies.
    However, ours with PME successfully localizes the motorcycle.
    }
    \label{fig:supple_qual_dark}
\end{figure*}

==> supple/image/supple_qual_occluded.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.95\textwidth]{supple/image/supple_qual_occluded.pdf}
    \caption{
    \textbf{Qualitative comparison of ours without PME and with PME.}
    Camera-only decoding branch fails to detect the pedestrian behind the traffic sign in the back left view camera.
    As a result, ours without PME misses the pedestrian due to the negative fusion, while ours with PME successfully localizes it.
    }
    \label{fig:supple_qual_occluded}
\end{figure*}

==> supple/sec/0.tex <==
% We provide a detailed PyTorch code of modality-agnostic decoding (MOAD) and proximity-based modality ensemble (PME) module in~\cref{supple:algorithm}.
In~\cref{supple:pme_analysis}, we compare modality ensemble strategies to validate the effectiveness of PME module.
Then, we provide additional qualitative results of MEFormer in~\cref{supple:qual} to further validate the effectiveness of PME in various environments.

==> supple/sec/1.tex <==
\section{Algorithm}
\label{supple:algorithm}

==> supple/sec/2.tex <==
\section{Analysis of PME}
\label{supple:pme_analysis}
\input{supple/table/ensemble_design}
In this section, we compare various modality ensemble strategies to validate the effectiveness of the PME module for modality ensemble.
Results are shown in Table~\ref{ensemble_design}.
For top-k and NMS, we aggregate all box predictions from three modality decoding branches and apply these strategies based on confidence scores, and they show significant performance degradation compared to ours without PME.
In addition, NME that does not use proximity-based attention mask $M$ also shows a 0.1\% mAP drop compared to ours without PME while ours with PME shows 0.13\% NDS and 0.14\% mAP enhancement.
This verifies that adaptively aggregating box features from three modality decoding branches using PME is effective for box refinement.

% Our PME module improves the detection performance of MEFormer in all environments.
% Especially for objects in a middle distance, there is a 0.24\% performance improvement.
% Also, on a rainy day, there is a performance improvement of 0.16\%.
% These results validate that the PME module prevents noisy information transfer in challenging environments.

==> supple/sec/3.tex <==
\section{More qualitative results}
\label{supple:qual}
\input{supple/image/supple_qual_occluded}
\input{supple/image/supple_qual_dark}
We validate the effectiveness of our PME module by comparing the qualitative results with and without PME.
In~\cref{fig:supple_qual_occluded}, the camera-only decoding branch fails to detect the pedestrian in the back left view camera since the traffic sign occludes the pedestrian.
As a result, ours without PME (\cref{fig:supple_qual_occluded}(a)) also misses the pedestrian due to the negative fusion problem.
However, ours with PME (\cref{fig:supple_qual_occluded}(b)) successfully detects the pedestrian by aggregating box features from the LiDAR decoding branch using PME module.
Additionally, from the front view camera in~\cref{fig:supple_qual_dark}, ours with PME (\cref{fig:supple_qual_dark}(b)) localizes the motorcycle, whereas without PME (\cref{fig:supple_qual_dark}(a)) fails to localize it even though the camera-only decoding branch detects it.
% Furthermore, in~\cref{fig:supple_qual2}, our framework without PME (\cref{fig:qual2_moad}) misclassifies the car in the back view camera as a truck.
% However, PME successfully classifies it as a car (\cref{fig:qual2_pme}).
These qualitative results show that the PME module prevents negative fusion during the modality fusion process.

==> supple/sec/4_tmp.tex <==
\input{supple/table/sensor_malfunction}

==> supple/table/ensemble_design.tex <==
\begin{table*}[t!]
\centering
\setlength{\tabcolsep}{20pt}
\begin{tabular}{lcc}
    \toprule
    Method & NDS & mAP \\
    % \midrule 
    \midrule
    Ours w/o PME & 73.66 & 71.25 \\
    % \midrule
    top-k ($k=300$) & 51.80 \scriptsize\textcolor{red}{($-21.86$)} & 33.34 \scriptsize\textcolor{red}{($-37.91$)} \\
    % NMS (IoU thres $=0.7$) & 61.59 & 52.43 \\
    NMS (IoU thres $=0.5$) & 63.86 \scriptsize\textcolor{red}{($-9.80$)} & 56.72 \scriptsize\textcolor{red}{($-14.53$)} \\
    % NMS (IoU thres $=0.3$) & 65.49 & 59.61 \\
    NME & 73.62 \scriptsize\textcolor{red}{($-0.04$)} & 71.15 \scriptsize\textcolor{red}{($-0.10$)} \\
    \midrule
    \textbf{PME} & \textbf{73.79} \scriptsize\textcolor{blue}{($+0.13$)} &\textbf{71.39} \scriptsize\textcolor{blue}{($+0.14$)} \\
    \bottomrule
\end{tabular}
\caption{
\textbf{Comparison of modality ensemble strategies.}
NME denotes naive modality ensemble which performs modality ensemble with no attention mask $M$ introduced in Eq. (9).
}
\label{ensemble_design}
\end{table*}


==> supple/table/image_blur.tex <==
\begin{table}[ht]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccc}
    \toprule
    Method & Modality & $k=5$ & $k=9$ & $k=13$ \\
    \midrule 
    \midrule
    PETR~\cite{liu2022petr} & C & 42.9 & 38.7 & 35.0 \\
    BEVFusion~\cite{liu2023bevfusion}$^\ast$ & L+C & 70.9 & 70.8 & 70.6 \\
    DeepInteraction~\cite{yang2022deepinteraction} & L+C & 69.0 & 68.8 & 68.5 \\
    SparseFusion~\cite{xie2023sparsefusion} & L+C & 72.7 & 72.4 & \textbf{71.9} \\
    CMT~\cite{yan2023cmt} & L+C & 72.5 & 71.7 & 71.0 \\
    \midrule
    Ours w/o PME & L+C & 73.1 & 72.4 & 71.5 \\
    \textbf{Ours} & L+C & \textbf{73.3} & \textbf{72.5} & 71.6 \\
    \bottomrule
\end{tabular}
}
\caption{
Detection performance with blurred images. We apply Gaussian blur with kernel size $k$ to images. $^\ast$ denotes the results obtained using the OpenPCDet~\cite{openpcdet2020} reproduced weights.
}
\label{image_blur}
\end{table}

% \begin{table}
% \centering
% \begin{tabular}{lccccccccc}
%     \toprule
%     \multirow{2}{*}{Method} & \multirow{2}{*}{Modality} & \multicolumn{2}{c}{$k=5$} & \multicolumn{2}{c}{$k=15$} & \multicolumn{2}{c}{$k=25$} & \multicolumn{2}{c}{$k=31$} \\
%     \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} & & NDS & mAP & NDS & mAP & NDS & mAP & NDS & mAP\\
%     \midrule 
%     \midrule
%     BEVFusion & L+C & - & - & - & - & - & - & - & - \\
%     CMT & L+C & 72.5 & 69.7 & 70.6 & \textbf{66.1} & 68.4 & \textbf{62.6} & 67.2 & 60.6 \\
%     \midrule
%     \textbf{Ours} & L+C & \textbf{73.3} & \textbf{70.2} & \textbf{71.1} & \textbf{66.1} & \textbf{68.9} & 62.4 & \textbf{67.9} & \textbf{60.7} \\
%     \bottomrule
% \end{tabular}
% \caption{
% image blur
% }
% \label{image_blur}
% \end{table}


==> supple/table/image_brightness.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{lccc}
    \toprule
    Method & Modality & +1 EV & -1 EV \\
    \midrule 
    \midrule
    PETR~\cite{liu2022petr} & C & 42.5 & 42.3 \\
    BEVFusion~\cite{liu2023bevfusion}$^\ast$ & L+C & 70.5 & 70.7 \\
    DeepInteraction~\cite{yang2022deepinteraction} & L+C & 68.5 & 68.7 \\
    SparseFusion~\cite{xie2023sparsefusion} & L+C & 72.1 & 71.6 \\
    CMT~\cite{yan2023cmt} & L+C & 72.1 & 72.3 \\
    \midrule
    Ours w/o PME & L+C & 72.2 & 72.6 \\
    \textbf{Ours} & L+C & \textbf{72.5} & \textbf{72.8} \\
    \bottomrule
\end{tabular}
\caption{
Detection performance according to various exposure value changes in the images. $^\ast$ denotes the results obtained using the OpenPCDet~\cite{openpcdet2020} reproduced weights.
}
\label{image_brightness}
\end{table}


==> supple/table/lidar_dropout.tex <==
\begin{table}[ht]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccc}
    \toprule
    Method & Modality & $p=0.2$ & $p=0.5$ & $p=0.8$ \\
    \midrule 
    \midrule
    Transfusion-L~\cite{Bai2022transfusion}$^\ast$ & L & 68.8 & 66.7 & 58.6 \\
    BEVFusion~\cite{liu2023bevfusion}$^\ast$ & L+C & 70.6 & 69.2 & 63.1 \\
    DeepInteraction~\cite{yang2022deepinteraction} & L+C & 68.7 & 67.4 & 62.3 \\
    SparseFusion~\cite{xie2023sparsefusion} & L+C & 72.4 & 71.0 & 65.5 \\
    CMT~\cite{yan2023cmt} & L+C & 72.6 & 71.7 & 68.2 \\
    \midrule
    Ours w/o PME & L+C & 72.9 & 72.0 & 68.5 \\
    \textbf{Ours} & L+C & \textbf{73.2} & \textbf{72.3} & \textbf{68.9} \\
    \bottomrule
\end{tabular}
}
\caption{
Comparison of detection performance under LiDAR malfunction scenarios. In this setting, we randomly drop points with probability $p$. $^\ast$ denotes the results obtained using the OpenPCDet~\cite{openpcdet2020} reproduced weights.
}
\label{lidar_dropout}
\end{table}

% \begin{table}
% \centering
% \begin{tabular}{lccccccc}
%     \toprule
%     \multirow{2}{*}{Method} & \multirow{2}{*}{Modality} & \multicolumn{2}{c}{p=0.2} & \multicolumn{2}{c}{p=0.5} & \multicolumn{2}{c}{p=0.8} \\
%     \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} & & NDS & mAP & NDS & mAP & NDS & mAP\\
%     \midrule 
%     \midrule
%     Transfusion-L* & L & 68.8 & 63.6 & 66.7 & 60.3 & 58.6 & 47.5 \\
%     BEVFusion* & L+C & 70.6 & 67.1 & 69.2 & 65.1 & 63.1 & 56.3 \\
%     DeepInteraction & L+C & 68.7 & 68.1 & 67.4 & 66.0 & 62.3 & 58.1 \\
%     SparseFusion & - & - & - & - & - & - \\
%     CMT & L+C & 72.6 & 69.8 & 71.7 & 68.6 & 68.2 & 63.8 \\
%     \midrule
%     \textbf{Ours} & L+C & \textbf{73.2} & \textbf{70.4} & \textbf{72.3} & \textbf{69.2} & \textbf{68.9} & \textbf{64.8} \\
%     \bottomrule
% \end{tabular}
% \caption{
% lidar dropout
% }
% \label{lidar_dropout}
% \end{table}


==> supple/table/lidar_sparsity.tex <==
\begin{table}[ht]
\centering
\caption{
Comparison of detection performance in sparse point clouds environment. $^\ast$ denotes the results obtained using the OpenPCDet~\cite{openpcdet2020} reproduced weights.
}
\label{lidar_sparsity}
\begin{tabular}{lcccc}
    \toprule
    Method & Modality & 16-beam & 4-beam& 1-beam\\
    \midrule 
    \midrule
    Transfusion-L~\cite{Bai2022transfusion}$^\ast$ & L & 58.9 & 49.6 & 22.2 \\
    BEVFusion~\cite{liu2023bevfusion}$^\ast$ & L+C & 63.0 & 55.3 & 30.4 \\
    DeepInteraction~\cite{yang2022deepinteraction} & L+C & 61.0 & 55.1 & 27.2 \\
    SparseFusion~\cite{xie2023sparsefusion} & L+C & 65.5 & 59.9 & 33.5 \\
    CMT~\cite{yan2023cmt} & L+C & 67.6 & 62.2 & 43.4 \\
    \midrule
    Ours w/o PME & L+C & 68.6 & 64.2 & 45.2 \\
    \textbf{Ours} & L+C & \textbf{68.8} & \textbf{64.7} & \textbf{45.8} \\
    \bottomrule
\end{tabular}
\end{table}

% \begin{table}
% \centering
% \begin{tabular}{lccccccc}
%     \toprule
%     \multirow{2}{*}{Method} & \multirow{2}{*}{Modality} & \multicolumn{2}{c}{16-beam} & \multicolumn{2}{c}{4-beam}& \multicolumn{2}{c}{1-beam}\\
%     \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} & & NDS & mAP & NDS & mAP & NDS &mAP\\
%     \midrule 
%     \midrule
%     Transfusion-L* & L & 58.9 & 46.1 & 49.6 & 31.8 & 22.2 & 2.7\\
%     BEVFusion* & L+C & 63.0 & 54.6 & 55.3 & 43.2 & 30.4 & 7.5\\
%     DeepInteraction & L+C & 61.0 & 55.6 & 55.1 & 46.0 & 27.2 & 8.3 \\
%     SparseFusion & L+C & 65.5 & 58.7 & 59.9 & 50.1 & 33.5 & 14.7 \\
%     CMT & L+C & 67.6 & 62.3 & 62.2 & 54.9 & 43.4 & 30.6\\
%     \midrule
%     \textbf{Ours} & L+C & \textbf{68.8} & \textbf{63.5} & \textbf{64.7} & \textbf{57.8} & \textbf{45.8} & \textbf{32.7}\\
%     \bottomrule
% \end{tabular}
% \caption{
% lidar sparsity. * denotes the results obtained using the OpenPCDet~\cite{openpcdet2020} reproduced weights
% }
% \label{lidar_sparsity}
% \end{table}


==> supple/table/sensor_malfunction.tex <==
\begin{table}[ht]
\centering
\caption{Robustness against noisy point clouds}
% \label{lidar_sparsity}
\begin{tabular}{lccccc}
    \toprule
    Method & Modality & 16-beam & 8-beam & 4-beam& 1-beam\\
    \midrule 
    \midrule
    Transfusion-L$^\ast$ & L & 58.9 & & 49.6 & 22.2 \\
    BEVFusion$^\ast$ & L+C & 63.0 & & 55.3 & 30.4 \\
    DeepInteraction & L+C & 61.0 & & 55.1 & 27.2 \\
    SparseFusion & L+C & 65.5 & & 59.9 & 33.5 \\
    CMT & L+C & 67.6 & & 62.2 & 43.4 \\
    \midrule
    Ours w/o PME & L+C & 68.2 &-  & 62.8 & - \\
    \textbf{Ours} & L+C &\textbf{68.9} & \textbf{-} & \textbf{63.3} & \textbf{41.6} \\
    \bottomrule
\end{tabular}
\end{table}


==> table/challenging_environment_table.tex <==
\begin{table*}[h!]
\centering
\setlength{\tabcolsep}{7pt}
\begin{tabular}{lccccc}
    \toprule
    \multirow{2}{*}{Method} &  \multirow{2}{*}{Modality} & \multicolumn{2}{c} {Night} & \multicolumn{2}{c} {Rainy} \\
    \cmidrule(lr){3-4} \cmidrule(lr){5-6}
    &  & NDS & mAP & NDS & mAP \\
    \midrule 
    \midrule
    PETR~\cite{liu2022petr}$\ddagger$ & C & 24.2 & 17.2 & 50.6 & 41.9 \\
    TransFusion-L~\cite{Bai2022transfusion}$\dagger$ & L  & 43.5 & 37.5 & 69.9 & 64.0 \\
    BEVFusion~\cite{liu2023bevfusion}$\dagger$ & L+C & 45.7 & 42.2 & 72.1 & 68.1 \\
    DeepInteraction~\cite{yang2022deepinteraction}$\ddagger$ & L+C & 43.8 & 42.3 & 70.6 & 69.4 \\
    \midrule
    CMT~\cite{yan2023cmt} & L+C & 46.3 & 42.8 & 73.7 & 70.5 \\
    \textbf{CMT w/ PME} & L+C & 46.3 & 43.0 & 74.0 & 70.7 \\
    \midrule
    \textbf{MOAD} & L+C & 46.6 & 43.1 & 74.6 & \textbf{72.2} \\
    \textbf{MOAD w/ PME} & L+C & \textbf{46.8} & \textbf{43.7} & \textbf{74.9} & \textbf{72.2} \\
    \bottomrule
\end{tabular}
\caption{
\textbf{Comparison of detection performance in challenging environments.}
$\dagger$ and $\ddagger$ denote the results obtained using the OpenPCDet~\cite{openpcdet2020} reproduced weights and weight provided in the official GitHub repository respectively.
}
\label{challenging_environment_table}
\end{table*}

